PillarTrack:Boosting Pillar Representation for Transformer-based 3D Single Object Tracking on Point Clouds

LiDAR-based 3D single object tracking (3D SOT) is a critical issue in robotics and autonomous driving. Existing 3D SOT methods typically adhere to a point-based processing pipeline, wherein the re-sampling operation invariably leads to either redundant or missing information, thereby impacting performance. To address these issues, we propose PillarTrack, a novel pillar-based 3D SOT framework. First, we transform sparse point clouds into dense pillars to preserve the local and global geometrics. Second, we propose a Pyramid-Encoded Pillar Feature Encoder (PE-PFE) design to enhance the robustness of pillar feature for translation/rotation/scale. Third, we present an efficient Transformer-based backbone from the perspective of modality differences. Finally, we construct our PillarTrack based on above designs. Extensive experiments show that our method achieves comparable performance on the KITTI and NuScenes datasets, significantly enhancing the performance of the baseline.

==> main.tex <==
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %2345678901234567890123456789012345678901234567890123456789012345678901234567890
% %        1         2         3         4         5         6         7         8

% \documentclass[letterpaper, 10 pt, conference]{ieeeconf}  % Comment this line out if you need a4paper
% % \usepackage[UTF8]{CJK}
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{xcolor}
% \usepackage{caption}
% \usepackage{url}
% \usepackage{epsfig} % for postscript graphics files
% \usepackage{mathptmx} % assumes new font selection scheme installed
% \usepackage{times} % assumes new font selection scheme installed
% \usepackage{amsmath} % assumes amsmath package installed
% \usepackage{amssymb}  % assumes amsmath package installed
% \usepackage{subfigure}
% \usepackage{array}
% \usepackage{color, soul}
% \usepackage[colorlinks,linkcolor=red,anchorcolor=blue,citecolor=green]{hyperref}
% \usepackage{booktabs}
% \usepackage{colortbl}
% \usepackage{tcolorbox}
% \usepackage{color,xcolor}
% \usepackage{multirow}
% \newcommand{\argmin}{\arg\!\min}
% \usepackage{float}
% \usepackage{cite}
% \usepackage{xcolor}
% \usepackage{algpseudocode}
% \usepackage[export]{adjustbox}
% \usepackage{balance}
% \usepackage{rotating}
% % \usepackage[utf8]{inputenc}
% \usepackage{graphicx}
% \def\eg{{\it e.g.}\xspace}
% \def\ie{{\it i.e.}\xspace}
% %\documentclass[a4paper, 10pt, conference]{ieeeconf}      % Use this line for a4 paper
% \usepackage[utf8]{inputenc}
% \IEEEoverridecommandlockouts                              % This command is only needed if 
%                                                           % you want to use the \thanks command

% \overrideIEEEmargins                                      % Needed to meet printer requirements.




% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \title{\LARGE \bf
% %PillarTrack: Redesigning Pillar-based Transformer Network for 3D Monocular Object Tracking in Point Cloud
% PillarTrack: Redesigning Pillar-based Transformer Network \\ for Single Object Tracking on Point Clouds}

% \author{Weisheng Xu$^{1}$$^\dagger$, Sifan Zhou$^{2}$$^\dagger$*, Zhihang Yuan% <-this % stops a space
% %\thanks{*This work was not supported by any organization}% <-this % stops a space
% \thanks{$^{1}$Weisheng Xu is with the School of Mathematics and Computer Science,
%         Nanchang University, Nanchang 330031, China.
%         {\tt\small 6105121101@email.ncu.edu.cn}, $^{2}$Sifan Zhou is with the School of Automation, Southeast University, Nanjing 210096, China.
%         {\tt\small sifanjay@gmail.com}, $^{3}$Zhihang Yuan is with Houmo AI,
%         Beijing 100088, China.
%         {\tt\small hahnyuan@gmail.com}}
% \thanks{$^\dagger$ Authors with equal contribution. * Corresponding author.}
% }
% \begin{document}
% \maketitle
% \thispagestyle{empty}
% \pagestyle{empty}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %resulting in underutilization of point cloud information.
% \begin{abstract}
% LiDAR-based 3D single object tracking (3D SOT) is a critical issue in robotics and autonomous driving. It aims to obtain accurate 3D BBox from the search area based on similarity or motion. However, existing 3D SOT methods usually follow the point-based pipeline, where the sampling operation inevitably leads to redundant or lost information, resulting in unexpected performance. To address these issues, we propose PillarTrack, a pillar-based 3D single object tracking framework. Firstly, we transform sparse point clouds into dense pillars to preserve the local and global geometrics. Secondly, we introduce a Pyramid-type Encoding Pillar Feature Encoder (PE-PFE) design to help the feature representation of each pillar. Thirdly, we present an efficient Transformer-based backbone from the perspective of modality differences. Finally, we construct our PillarTrack tracker based above designs. Extensive experiments on the KITTI dataset demonstrate the superiority of our proposed method. Notably, our method achieves state-of-the-art performance on the KITTI dataset and enables real-time tracking speed. We hope our work could encourage the community to rethink existing 3D SOT tracker designs. 



% %Moreover, we find that by simply integrating existing advanced network designs, rather than complex network architecture designs, it is easy to achieve state-of-the-art results in LiDAR-based 3D SOT tasks. Therefore, we also encourage the community to draw much inspiration from advanced designs and rethink existing 3D tracker designs.


% %LiDAR-based 3D single object tracking finds extensive applications in robotics and autonomous driving. However, the sparsity inherent in point clouds poses significant challenges in tracking under occlusion and long-range scenarios. Consequently, effective extraction of global representations from sparse input point clouds is of paramount importance. To address these challenges, we propose a novel 3D single object tracking framework based on a transformer architecture with a pillar representation. Firstly, we convert sparse point clouds into dense pillar features in the Bird's Eye View (BEV) projection and introduce a pyramid-level Pillar encoding structure to enhance the feature representation. Subsequently, we reexamine the existing transformer architecture design from the perspective of modality differences and present an efficient transformer encoder tailored for point cloud tracking tasks. Furthermore, we provide a range of scalable encoder networks based on this design for different runtime requirements. Lastly, we integrate state-of-the-art neural network designs and present a 3D tracker that meets various speed and accuracy demands. Extensive experiments conducted on the KITTI dataset demonstrate the superiority of our proposed method, achieving state-of-the-art results. Notably, our method attains SOTA performance on the KITTI dataset and enables real-time tracking models to accommodate diverse runtime constraints. Moreover, we find that by integrating and adapting existing advanced network designs, it is possible to achieve SOTA results, thereby encouraging the community to seek inspiration from advanced structural designs and reassess existing 3D tracker designs.

% %LiDAR-based 3D Single Object Tracking is a critical issue in the fields of robotics and autonomous driving. Current methods typically focus on enhancing model performance, often neglecting the consideration of real-time capabilities. In this paper, we revisit the application of three-dimensional point cloud processing in object tracking from the perspective of resource allocation, while comprehensively considering both accuracy and latency. Our research reveals that even the most basic pillar-based models can exhibit surprisingly excellent performance. Moreover, our analysis indicates that adjusting the number of channels and the hierarchical structure of the point cloud processing network significantly impacts model performance. Through extensive experimental validation, our pillar-based network, combined with modern architectural design and training strategies, has demonstrated industry-leading performance on the widely recognized benchmarks KITTI and nuScenes. Our results suggest that traditional grid-based methods for geometric modeling of point cloud data may be overestimated in their contribution to 3D object detection performance. Additionally, our study confirms that adopting modern network structure designs plays a decisive role in enhancing model performance and adaptability in the field of 3D single object tracking.
% % \begin{figure}[t]
% % 	\includegraphics[width=0.99\linewidth]{fig/model_size.pdf}
% % 	% \hspace{-44mm}\resizebox{.46\columnwidth}{!}{\tablestyle{2pt}{1}
% %         \hspace{-33mm}\resizebox{.38\columnwidth}{!}{
% % 		\begin{tabular}[b]{l|cr}
% %                 % \toprule
% % 			& mAP & \#Params  \\
% %                 \hline
% % 			CP-Pillar \cite{centerpoint} & 50.3\%  & 6.0M \\
% % 			\bf \cnn{}-Tiny & \bf 58.8\%  & \bf 0.6M\\
% % 			\hline
% % 			CP-Voxel~\cite{centerpoint} & 57.6\% & 9.5M \\
% % 			\bf \cnn{}-Small & \bf 61.7\%  & \bf 2.7M \\
% % 			\hline
% %                 PillarNet~\cite{PillarNet}  &  60.2\% & 17.1M \\
% %                 \bf \cnn{}-Base & \bf 63.2\% & \bf8.9 M \\
% % 			\hline
% %                 FastPillar~\cite{FastPillars}   & 61.7\% & 11.6M \\
% % 			\bf \cnn{}-Large & \bf 64.3\% & \bf 12.3M \\
% %                 % $^\dagger$
% % 			% \multicolumn{3}{l}{~~$^\dagger$Not plotted ~~\vspace{15mm} } \\
% %                 \vspace{16mm} \\ % \vspace{-3mm}
% %                 % \bottomrule
% % 	\end{tabular}}
% %     \vskip -0.15in
% % 	\caption{\textbf{Model Size vs. mAP.} All results are reported with a single model in nuScenes val set. CP: CenterPoint.}
% % 	\label{fig:model_size}
% % \end{figure}  
% % \end{CJK*}
% \end{abstract}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \section{INTRODUCTION}
% % \begin{CJK*}{UTF8}{gbsn}
% %这里参考PTT/M2-track来叙述3DSOT的重要性，一步步引出3D SOT 任务。
% %尽管已有广泛的研究致力于专门开发针对这一领域的复杂网络架构，如通过引入区域提议网络（RPN）[2]和点云卷积网络（PointNet）等先进技术，但这些方法往往依赖于对点云进行预处理，如体素化或投影到二维平面，这可能会损失宝贵的几何信息。
% %要陈述point-based的方法部署困难，且感受野有限，不如dense的方式有更多的信息保留，同时transformer-based的方法目前有着全局感受野，展现出更惊人的效果。我们的目的是从参数有效的和面向实际部署考虑的角度出发，探索更高效的高性能transformer-based的点云跟踪网络，希望通过一系列经验研究和实验设计，给研究社区一定的启发和帮助。
% %3D单目标跟踪应用广泛，有哪些应用，为什么需要这个任务。然后陈述这个任务是要干什么的，现有方法的优缺点。借着陈述这些优越点会带来什么影响。最后陈述我们的方法，参考摘要，给出贡献。
% %贡献。1. PyramidPillar 2.modality-based transformer. 3. empirical advanced design and sota performance. 

% %Single object tracking (SOT) is a fundamental problem in computer vision with diverse applications in autonomous driving\cite{robust-tracking, FaF, pointtracknet} and robotics\cite{Trackingpeople,JMDT, Online}. %Over the past few years, substantial efforts\cite{SiamFC,VOT18,SiameseRPN,SiamMask} have been dedicated to 2D object tracking from RGB data. leveraging prevalent Siamese network architectures. In addition to visual sensors, 3D LIDAR sensors are now widely used in mobile robots or drones \cite{tartandrive,zhao2023subt}. Compared to 2D images, LiDAR point clouds exhibit greater robustness against illumination change and provide more accurate distance measurements, promoting the attention towards LiDAR-based 3D single object tracking \cite{sc3d,cui2019point,fang20203d}. Given the initial state (appearance and location) of specific target in the first frame, 3D single object tracking aims to estimate its 3D state across subsequent frames.

% 3D Single object tracking (3D SOT) has a diverse applications in autonomous driving and robotics. Given the initial state (appearance and location) of specific target in the first frame, 3D single object tracking aims to estimate its 3D state across subsequent frames. Existing LiDAR-based 3D single object tracking methods~\cite{fang20203d,p2b,ptt,bat,lttr,zhou2022pttr,hui2022stnet} generally follow the Siamese paradigm from 2D visual object tracking, aiming to achieve a trade-off between runtime and accuracy. Given the sparse and irregular input point cloud, these methods initially leverage PointNet families~\cite{qi2017pointnet, qi2017pointnet++} to learn point-wise discriminative representation, and then obtain point-wise similarity with a feature aggregation module. Finally, they estimate the state of specific targets based on these similarity features. SC3D \cite{sc3d} stands as the pioneering LiDAR-based 3D Siamese tracker, leveraging an efficient auto-encoder based on PointNet\cite{pointnet} for point-wise feature encoding. Subsequently, approaches such as P2B~\cite{p2b}, 3D-SiamRPN\cite{fang20203d}, BAT~\cite{bat} and PTT~\cite{ptt,ptt-journal} employ PointNet++~\cite{qi2017pointnet++} to extract more effective point-wise representation and achieve superior tracking performance. However, one common issue with above point-based 3D SOT methods is the need for re-sampling the input points to a fixed number. For instance. P2B~\cite{p2b} requires the input points to be re-sample to 1024 for the search area and 512 for the template point cloud in order to align the network input. This re-sample operation inevitably introduces the potential for redundant or lost information, which can adversely affect performance. Additionally, the reliance on point query/retrieval in 3D space (e.g., PointNet++ \cite{qi2017pointnet++}) for the re-sampling process may not be friendly to efficient hardware implementation. 
% \begin{figure}[t] 
%   \centering
%   \includegraphics[width=\linewidth]{figures/Speed-Preci.pdf}
%   \caption{Comparison with other 3D SOT methods on KITTI dataset. We categorize methods based on the Backbone architecture and report their performance on Success and Precision.}
%   \label{performance}
%   \vspace{-4mm}
% \end{figure}


% To this end, inspired by the recent advancements in pillar-based 3D object 
% detectors~\cite{shi2022pillarnet,zhou2023fastpillars,pillarnext} due to their real-time
% speed and high performance. Therefore, we convert the sparse and irregular point clouds
% into dense and regular pillar representations. It is noteworthy that the 3D SOT task 
% can be regarded as a specific 3D object detection task within a local search area, with 
% the additional template point prior information. Therefore,it is natural to leverage 
% advanced principles from 3D point cloud detection to improve point cloud tracking 
% tasks. Specifically, pillar-based point cloud representation possesses following 
% advantages:\textbf{(1)} Pillar representation is dense and ordered, facilitating 
% seamless integration with advanced 2D image-based techniques without much modification. 
% \textbf{(2)} The compact nature of the pillar representation reduces computational 
% overhead while maintaining a desirable trade-off between performance and speed. 
% \textbf{(3)} Pillar representation is deployment-friendly, making it highly suitable 
% for resource-limited devices like mobile robots or drones. Particularly,pillar 
% representation naturally aligns with the high demanding real-time requirements of 3D 
% trackers, making it well-suited for tracking tasks.

% Currently, few works~\cite{smat,pttr_journal} are dedicated to pillar-based 3D SOT with point clouds. SMAT~\cite{smat} addresses this gap by transforming sparse 3D point clouds into dense pillars and then utilizing a transformer-based encoder for multi-scale feature extraction and interaction, yielding promising results. However, SMAT directly adopts a simplistic pillar encoding module from PointPillars~\cite{pointpillars} limits the quality of the pillar representations. Besides, their backbone directly follows the design principle of vision transformers tailored for RGB image, which may be sub-optimal for point cloud modalities. PTTR++~\cite{pttr_journal} introduces a fusion of point-wise and pillar-wise views to further enhance the performance of PTTR~\cite{zhou2022pttr}. Nevertheless, PTTR++ still involves a re-sampling operation within its pipeline, which presents paratical deployment challenges. 

% In this paper, we propose PillarTrack, a pillar-based 3D single-object tracking framework, aiming to improve tracking performance while enhancing the inference speed. Firstly, we transform sparse and unordered point clouds into dense and regular pillar representations to reduce information loss caused by re-sampling operation and propose a Pyramid-type Encoding Pillar Feature Encoder (PE-PFE) design to help the feature learning of each pillar. Secondly, we argue the design of existing Transformer-based backbone from the perspective of modality differences and propose an modality-aware Transformer-based backbone specifically tailored for point cloud modalities, achieving higher performance with fewer GFLOPs. Finally, we construct our PillarTrack network. Extensive experiments on the KITTI dataset demonstrate the superiority of our proposed method. As shown in Figure ~\ref{performance}, our approach achieves state-of-the-art performance on the KITTI dataset, striking a better balance between speed and accuracy, and catering to diverse practical needs. In conclusion, the main contributions of this paper are as follows:

% %Moreover, we find that by simply integrating existing advanced network designs, rather than complex network architecture designs, it is easy to achieve state-of-the-art results in LiDAR-based 3D SOT tasks. Therefore, we also encourage the community to draw much inspiration from advanced designs and rethink existing 3D tracker designs. Overall, the main contributions of this paper are as follows:




% $\bullet$ \textbf{PE-PFE}: A Pyramid-type Encoding Pillar Feature Encoder (PE-PFE) design to encode the point coordinate of each pillar with pyramid-type representation, and bring the performance gain without extra computational overhead.

% $\bullet$ \textbf{Modality-aware Transformer-based Backbone}: A more suitable for point cloud modalities, aiming to enhance feature representation. This design involves a simple adjustment of computational resources allocated to the front-end of the backbone, allowing for capturing more semantic details of the input point cloud.

% $\bullet$ \textbf{SOTA and Open-source}: Experiments on KITTI dataset show our method achieve the state-of-the-art performance. Besides, we will open source our code to the research community in \url{https://github.com/StiphyJay/PillarTrack}.

% %However, despite some progress in handling point cloud data, these grid-based conversion methods have not been thoroughly experimentally verified and optimized in terms of model performance and inference latency. The pillar-based approach inevitably introduces information loss when processing point clouds, which is particularly evident when tracking small objects like pedestrians, leading to a degradation in tracking performance. In contrast, the voxel-based method retains more point cloud information, thereby enhancing the tracker's performance to a certain extent. Nevertheless, this method requires more computational resources, which not only increases the model's inference latency but also limits its practicality in real-time applications. Different point cloud conversion strategies naturally correspond to their most suitable network architecture designs, which necessitate that we consider the adaptability between point cloud characteristics and network structure when designing tracking models.

% %We have observed that the current research trend in 3D single object tracking (SOT) is gradually shifting towards the development of more specialized operators and the exploration of contextual semantic relationships within point clouds. In the field of 3D SOT, 3D object detection serves as the cornerstone for subsequent semantic processing, yet the optimization of network computational architecture has received little in-depth discussion. Most existing studies are still based on primitive architectures built upon early works such as PointNet\cite{pointnet} or BEV\cite{}, which lack modern design elements like powerful backbone networks, effective feature fusion strategies, and improved training methods—key factors that have led to significant advancements in the field of 2D object detection.\\

% %Concurrently, in the closely related field of 2D object detection, we have witnessed significant technological advancements, largely attributable to innovations in network architecture and optimization of training strategies. These advancements include, but are not limited to, powerful backbone networks (such as ResNet\cite{he2016deep} and Swin Transformer\cite{liu2021swin}), efficient feature fusion modules (e.g., YOLOF\cite{chen2021you}), and innovative training strategies (e.g., Bag of Freebies\cite{zhang2019bag}). These achievements have led to notable breakthroughs in the field of 2D object detection. In contrast, research in 3D object detection has largely continued to employ early methods and lacks similar modern design elements.

% %Based on these observations, we have reevaluated the focus of our research on 3D object detection within LiDAR point clouds, particularly delving into the design of local point aggregators and network architecture. In our in-depth analysis of local point aggregators, we introduce a new perspective—computational budget. This perspective allows us to more accurately assess the efficiency of different aggregators in terms of resource allocation. Specifically, fine-grained aggregators, such as voxel-based methods, typically require more computational resources because they rely on 3D convolutions, which not only increases the number of network parameters but also significantly reduces processing speed. In contrast, pillar-based aggregators maintain high operational efficiency while achieving performance comparable to or even surpassing that of voxel-based aggregators. As shown in Figure 1, under the same computational budget and optimized training strategies, pillar-based models demonstrate competitiveness across multiple key performance metrics. This challenges our traditional understanding of the role of fine-grained structures in enhancing performance and prompts deeper contemplation on how to achieve optimal performance with limited computational resources. Our research findings indicate that with carefully designed network architectures and training strategies, even simple pillar-based models can achieve or exceed the performance of complex voxel-based models in 3D object detection tasks. This provides a new direction for future research in 3D object detection under resource-constrained environments.

% %Secondly, we conducted an in-depth exploration of network architecture design, particularly focusing on the optimization requirements for channel structures and layer structures in response to different point cloud conversion methods. We found that voxel-based point cloud conversion methods can achieve significant performance improvements when equipped with wider channels and an appropriate number of layers. This suggests that to fully leverage the high-density information of voxelized point clouds, the network needs to have sufficient parameters and computational depth to capture complex spatial features. On the other hand, pillar-based point cloud conversion demonstrates efficiency within a relatively streamlined network structure, indicating that the pillar structure can effectively aggregate point cloud features with fewer computational resources. Our research results emphasize the importance of customizing the channel and layer configurations of the network according to the adopted point cloud conversion strategy to achieve the best balance of performance and efficiency in the design of 3D object detection networks.

% %Based on our research findings, we designed and implemented a pillar-based network architecture named PillarBest, which achieves a perfect match with the pillar transformation method through optimized channel counts and layer structures. PillarBest not only achieved state-of-the-art tracking performance on the widely recognized benchmarks of KITTI\cite{kitti} and nuScenes\cite{nuscenes} but also demonstrated its efficiency in practical applications. Concurrently, we developed a highly adaptable network architecture, which, although ranked second in performance, achieved optimal inference latency, and we named it the xx network. The introduction of this network architecture provides new possibilities for achieving low-latency processing while maintaining high performance, especially in resource-constrained real-time application scenarios. Our approach is simple yet effective and possesses strong scalability and versatility.

% %By carefully designing point cloud conversion strategies and optimizing network structures, we have developed a series of detection networks that effectively balance detection accuracy and inference latency, making them particularly suitable for real-time object tracking applications in autonomous driving systems. These networks not only provide high-precision object detection but also ensure efficient operation in resource-constrained environments, offering reliable perceptual capabilities for autonomous vehicles.

% %Our main contributions can be summarized as follows: First, we explored the deep matching relationship between different point cloud conversion methods and network structures, revealing how to optimize network design to adapt to specific point cloud representations. Second, we considered both performance and inference latency in model design, ensuring that the model maintains high accuracy while also being scalable and adaptable, which is crucial for real-time application scenarios such as autonomous driving. Lastly, the xx model we proposed has achieved state-of-the-art performance (SOTA) on both the KITTI and nuScenes authoritative test sets, not only validating the effectiveness of our methods but also providing new research directions and practical benchmarks for the field of 3D single object tracking.
% % \end{CJK*}

% % 

% \section{Related Work}

% \subsection{Single Object Tracking on Point Clouds}
% Benefiting from the nature of LiDAR that are less sensitive to illumination changes and capture accurate distance information, numerous works\cite{sc3d, cui2019point, FSiamese, fang20203d, p2b, bat, mmtrack, v2b} in LiDAR-based 3D Single Object Tracking (3D SOT) have merged. SC3D\cite{sc3d} leverages the Kalman filter for proposals generation and select the most suitable candidate based on Siamese network\cite{bertinetto2016fully}. 3D-SiamRPN \cite{fang20203d} combines 3D Siamese network with 3D RPN network for object tracking. P2B\cite{p2b} introduces target-specific features and utilizes VoteNet\cite{votenet} to estimate target center. Based on the P2B pipeline, BAT\cite{bat} incorporated Box-aware information to enhance similarity feature. Besides, V2B\cite{v2b} introduces Voxel-to-BEV network for pixel-wise regression of 3D targets, M2-Track \cite{mmtrack,zheng2023effective} adopts a motion-centric paradigm to address the issue of 3D SOT and achieves remarkable performance. Inspired by the success of transformers\cite{vaswani2017attention}, several methods \cite{ptt, ptt-journal,lttr, zhou2022pttr, guo2022cmt, hui2022stnet, tat, xu2023cxtrack} have merged. PTT \cite{ptt,ptt-journal} proposed Point-Track-Transformer module to assign weights to crucial point cloud features. LTTR\cite{lttr} proposes a Transformer-based feature fusion module to learn semantic context among different region. PTTR\cite{zhou2022pttr} employs an attention-based feature matching mechanism to integrate target clues in similarity. STNet\cite{hui2022stnet} develops an iterative coarse-to-fine correlation network for robust correlation learning. CXTrack\cite{xu2023cxtrack} adopts transformer to extract richer contextual information from consecutive frames, enhancing localization accuracy. Recently, SMAT\cite{smat} encodes global similarity based on attention in the BEV to alleviate the impact of point sparsity. However, their backbone still partially inherits the design principles from ResNet\cite{resnet} tailored for the image modality, which may be sub-optimal for point clouds modality.


% \begin{figure*}[!htbp]
% \centering
% \includegraphics[width=0.9\textwidth]{figures/pipeline.pdf}\vspace{-2mm}
% \caption{The architecture of our PillarTrack network.Given the template and search area, we first use PE-Pillar to extract multi-scale features respectively. Then, MAE computes similarity by attention at each feature scale and then fuses the multi-scale similarity feature.Finally, we apply the detection head on the feature fusion map to localize the target.}
% \label{fig:num_blocks}
% \vspace{-3mm}
% \end{figure*}

% \subsection{Pillar-based Object Detection on Point Clouds}
% Grid-based point cloud 3D detectors\cite{pointpillars,yin2021center, shi2022pillarnet, zhou2023fastpillars, pillarnext} generally transform unordered points into regular pillar/voxel and then utilize 2D/3D CNN to learn representation. VoxelNet~\cite{zhou2018voxelnet} stands as a pioneering work that leverages Voxel Feature Extractor (VFE) and 3D CNN for 3D object detection. Subsequently, SECOND~\cite{yan2018second} employs 3D sparse convolution on non-empty voxels to accelerate training and inference. Different from above approaches, PointPillars~\cite{pointpillars} innovatively converts point clouds into pillars and leverages 2D CNN to enhance detection speed. After that, CenterPoint\cite{yin2021center} proposes a center-based head design, achieving milestone performance. Furthermore, PillarNet\cite{shi2022pillarnet} improves the accuracy of pillar-based 3D detectors through an "encoder-neck-head" architecture, achieving superior performance while maintaining real-time speed. Based on PillarNet\cite{shi2022pillarnet}, FastPillars\cite{zhou2023fastpillars} proposes a backbone design suitable for point cloud modality and considers deployment-friendly ability, resulting in new state-of-the-art. The success of these pillar-based 3D detectors greatly motivates us to explore the potential of simple pillar-based representation in 3D SOT tasks.
% %Recently, PillarNext\cite{li2023pillarnext} achieves promising accuracy through a series of designs, including increasing the neck's receptive field. 


% \subsection{Vision Transformer}
% Transformer\cite{vaswani2017attention} is first proposed in natural language processing (NLP). Subsequently, owing to its remarkable ability for global modeling, the Transformer has shown significant success in image recognition tasks. ViT\cite{vit} leverage the Transformer structure to classify images by splitting them into patches. SwinTransformer\cite{swin} proposes a shifted windows attention mechanism, achieving excellent performance across various image tasks. PVT\cite{pvt} and PVTv2\cite{pvtV2} utilize a progressive shrinking pyramid to construct a visual Transformer backbone. In the 3D Vison, Point Transformer\cite{zhao2021point} introduces a specialized Point Transformer layer tailored for processing unordered point clouds. PCT\cite{guo2021pct} utilizes 3D coordinates of points to generate position embedding and employs an attention module to extract point features from local neighborhoods. These efforts showcase outstanding performance in point cloud shape classification or part segmentation. For LiDAR-based 3D detection tasks, recent approaches\cite{sst,liu2023flatformer} first transform point clouds into regular pillars/voxels and then utilize dynamic sparse windows on BEV feature for feature extraction, yielding remarkable performance. In contrast, we employ the Transformer for global modeling on the pillarized feature, aiming to explore the potential of the Transformer in the object tracking task from a BEV perspective.

% %Additionally, In the dense prediction, DETR\cite{detr} first applies the transformer to object detection and deals with the detection problem as a set of predictions to match object queries based on the attention module. Deformable-DETR\cite{zhu2020deformable} further proposes multi-scale deformable attention module to speed up the convergence of DETR and achieve better performance.

% \section{Preliminary}
% \subsection{Problem Statement} 
% %这里参考https://arxiv.org/pdf/2207.11995.pdf 这篇文章的3.1，把3D SOT问题的定义写出来。把下面两段英文做一下整合即可

% % A 3D BBox is represented as $(x, y, z, w, l, h, \theta) \in \mathbb{R}^7$, where $(x, y, z)$ stands for the coordinate of the BBox center, $(w, l, h)$ is the BBox size and $\theta$ is the heading angle (the rotation around the up-axis). A point cloud is represented as $\{p_i\}_{i=1}^N$, where each point $p_i$ is a vector of its $(x, y, z)$ coordinate and $N$ is the number of points.

% % In 3D single object tracking (SOT), the BBox of the target in the first frame is given to the tracker. The goal of the tracker is to consistently localize the same target across consecutive frames. Notice that in the 3D case, any BBox is amodal (covering the entire object even if only part of it is visible). A template point cloud $P_t = \{p_{t_i}\}_{i=1}^{N_t}$ is generated by cropping and centering the target in the first frame with the given BBox $B_t$. For any search area $P_s = \{p_{s_i}\}_{i=1}^{N_s}$ in other frames, previous trackers take in the pair $(P_t, P_s)$ and output the amodal BBox of the target in the search area.

% % Formally, trackers can be formulated as:
% % \begin{equation}
% % \text{track} : \mathbb{R}^{N_t \times 3} \times \mathbb{R}^{N_s \times 3} \rightarrow \mathbb{R}^4, \quad (1)
% % \end{equation}
% % \begin{equation}
% % \text{track}(P_t, P_s) \rightarrow (x, y, z, \theta). \quad (2)
% % \end{equation}

% % Note that the output has only 4 elements since we do not need to re-predict the size of the 3D BBox, which is unchanged across all frames. Since previous works compare the search area only with the template that is usually incomplete, they lack the ability to capture the size and part information of the target object. Therefore, they are prone to produce false target proposals when similar objects are present. In this work, we aim at designing a box-aware tracker $\text{track}_{\text{box-aware}}$ that exploits the amodal BBox of the target:

% % \begin{equation}
% % \text{track}_{\text{box-aware}} : \mathbb{R}^7 \times \mathbb{R}^{N_t \times 3} \times \mathbb{R}^{N_s \times 3} \rightarrow \mathbb{R}^4, \quad (3)
% % \end{equation}
% % \begin{equation}
% % \text{track}_{\text{box-aware}}(B_t, P_t, P_s) \rightarrow (x, y, z, \theta). \quad (4)
% % \end{equation}

% %Additionally, we have a set of objects in the 3D scene $\mathbf{B}=\{\mathbf{b}_j=[x_j, y_j, z_j, h_j, w_j, l_j, {\theta}_j, c_j]^T \in \mathbb{R}^{M \times 8}\}$, where $M$ is the total number of objects, and $\mathbf{b}_i$ represents the $i$-th object in the scene. The coordinates $x_j, y_j, z_j$ indicate the object's center, while $h_j, w_j, l_j$ denote its size, ${\theta}_j$ is the object's heading angle, and $c_j$ represents the object's class. The core task of LiDAR-based 3D object detection is to accurately identify these 3D boxes $\mathbf{B}$ from the point cloud $\mathbf{P}$.

% In the task of the 3D Single Object Tracking (3D SOT), we initially define target point cloud (i.e., template) $\mathbf{P_t}=\{\mathbf{p}_{ti}=[x_i, y_i, z_i, r_i]^T \in \mathbb{R}^{N \times 4}\}$, where $x_i, y_i, z_i$ denote the coordinate values of each point along the axes X, Y, Z, respectively, and $r_i$ represents the laser reflection intensity. Our goal is to locate the the 3D bounding box (3D BBox) of this target in the search area $\mathbf{P_t}=\{\mathbf{p}_{si}=[x_j, y_j, z_j, r_j]^T \in \mathbb{R}^{M \times 4}\}$ frame by frame. Here, $N$ and $M$ is the number of points in target and search area. The 3D BBox is represented as $\mathbf{B}=\{\mathbf{b}=[x, y, z, h, w, l, {\theta}]^T \in \mathbb{R}^{1 \times 7}\}$, The coordinates $x, y, z$ indicate the object's center, while $h, w, l$ denote its size, ${\theta}_j$ is the object's heading angle. Since the target's 3D BBox is known in the first frame, we need to regress the target center and heading angle in subsequent frames. By applying the displacement and heading angle from the previous frame's 3D BBox, we can locate the target in the current frame.
% \vspace{-2mm}
% \subsection{Baseline Architecture Overview}
% As SMAT represents the first attempt at a pillar-based 3D Siamese tracker and has shown promising performance, we choose SMAT as our baseline and provide a brief overview of its structure. The core components of SMAT include: \textbf{1)} a naive pillar feature encoding module derived from Pointpillars, which transforms raw point cloud data into a pseudo-image; \textbf{2)} a Transformer-based backbone network that computes similarity through a multi-head attention mechanism for the multi-scale features from both the template and search branches, capturing local and global information within the point cloud; \textbf{3)} a neck module that integrates features from different scales and fuses multi-scale similarity features, enhancing the model's perception of multi-scale information; \textbf{4)} a decoder that predicts the position and orientation of the target object. These carefully designed features enable SMAT to effectively handle sparse point cloud data, offering an efficient solution for 3D Single Object Tracking.

% \subsection{Motivation}
% Our research endeavors to investigate a real-time, high-performance, pillar-based approach for 3D single-object tracking. To achieve this, we leverage the compact pillar representation and design a strong Transformer-based backbone that enhances pillar feature representation with reduced computational resources from the perspective of modality differences. Regarding the feature integration and similarity computation module, we follow the original design of baseline method\cite{smat}, which has shown remarkable efficacy. We hope that our design principles offer a novel perspective in 3D single object tracking, encouraging the community to revisit existing methodologies.
% %To achieve this, we employ a neural network to process the input point cloud with $M$ points. The network outputs a subset of the input containing N interest points (seeds) $S=\left\{s_i\right\}^{N}_{i=1}$, where each seed $s_i=(c_i,f_i)$ is composed of a 3D coordinate vector $c_i$ and a D-dimensional descriptor $f_i$ of the local object geometry. Our goal in utilizing the Transformer is to perform an attention-weighted operation on the feature space of $f_i$, yielding refined features $f_i^*$ with the same dimension. This approach enables us to more accurately capture and track changes in the target object across consecutive frames.

% % \subsection{Base Architecture Overview}

% \section{Method}

% \subsection{Pyramid-Encoded Pillar Feature Encoding Design} 

% \begin{figure}[!htbp]
% \centering
% \includegraphics[width=0.9\linewidth]{figures/QApillar.pdf}
% % Reduce the figure size so that it is slightly narrower than the column.
% \caption{The illustration of PE-PillarVFE design. We encode the channel information of the input point cloud in a pyramid-type fashion. This Pyramid-type encoding design allows the network to optimize more effectively without the input information loss.}
% \label{fig:PE-PFE}
% \vspace{-4mm}
% \end{figure}

% In pillar-based 3D detection methods\cite{pointpillars,shi2022pillarnet,zhou2023fastpillars}, Pillar Feature Encoding (PFE) plays a crucial role, directly impacting the representation learning of BEV feature and final detection accuracy. Its significance extends to 3D single object tracking tasks as well. In SMAT, they utilize the PFE module from PointPillars~\cite{pointpillars} to extract pillar-wise feature. Here, taking PFE module as an example, we illustrate the details of their input encoding. The points in each pillar are initially concatenated along the channel dimension to form $\hat{p_i}=\{[x_i, y_i, z_i, r_i,  {x}_{i}^{m}, {y}_{i}^{m}, {z}_{i}^{m}, {x}_{i}^{c},{y}_{i}^{c}, {z}_{i}^{c}] \in {\mathbb{R}^{N_v \times 10}} \}$, where $[x_i, y_i, z_i]$ is the original point coordinates in the ego frame, $[{x}_{i}^{m}, {y}_{i}^{m}, {z}_{i}^{m}]$ denotes the offset of $p_i$ from the mean of the xyz coordinates of all points within the current pillar, and $[{x}_{i}^{c},{y}_{i}^{c}, {z}_{i}^{c}]$ is the offset of $p_i$ from the current pillar center. However, there exist significant numerical differences in the point-wise feature. For example, the numerical range of the $[x_i, y_i, z_i]$ is $[-3.2,3.2]$ (i.e., the range of search area). However, the numerical range of $[{x}_{i}^{m}, {y}_{i}^{m}, {z}_{i}^{m}]$ and $[{x}_{i}^{c},{y}_{i}^{c}, {z}_{i}^{c}]$ is $[-0.1, 0.1]$, since they are relative offset within a pillar. It can be observed that there exist significant numerical differences (almost 30 $\times$) between the point-wise feature channels in PFE. Such huge disparities in input values pose significant challenges for network optimization ~\cite{glorot2010understanding, santurkar2018does}. Therefore, we propose a Pyramid-type Encoding Pillar Feature Encoder (PE-PFE) design aimed at reducing the numerical differences between the input channels, enabling the network towards better optimization on numerically stable inputs. 

% \begin{table}[h]
% \centering
% \caption{Tracking performance comparison of different PFE designs in the Car category in KITTI.}
% \resizebox{0.8\linewidth}{!}{
% \centering
% \begin{tabular}{c|c|c}\toprule[.02cm]
% PFE Method & Success & Precision \\ %&Success$_{BEV}$\\
% \toprule %3463-64-128-320-512-
% PFE (SMAT \cite{smat}\footnotemark[3])     & 68.9  & 79.6 \\
% PE-PFE(Ours)  & 70.8 (\textbf{+1.9})  & 80.3 (\textbf{+0.7}) \\ 
% \bottomrule
% \end{tabular}
% }
% \label{table:pepfe}
% \vspace{-2mm}
% \end{table}
% \vspace{-2mm}
% \begin{figure}[!htbp]
% \centering
% \includegraphics[width=0.8\linewidth]{figures/LOSS_total_new.pdf}
% % Reduce the figure size so that it is slightly narrower than the column.
% \caption{The loss comparison of different PFE designs.}
% \label{fig:PE-loss}
% \vspace{-2mm}
% \end{figure}
% \footnotetext[3]{The model was trained on a setup comprising four NVIDIA GeForce RTX 3090 GPUs}
% As shown in Figure \ref{fig:PE-PFE}, we encode the channel values of the input point cloud in a pyramid-type manner, and finally retain a residual value that cannot be evenly divided. The encoding values from each layer and the residual value are then cascaded together as point-wise features, which are then processed by the PFE module. It is important to note that this pyramid-type encoding design significantly reduces the numerical differences between the input data channels without sacrificing the information contained in the point cloud. This design helps the network achieve better optimization results. Furthermore, to demonstrate the effectiveness of our PE-PFE design compared to the naive PFE from PointPillars~\cite{pointpillars}, we present the performance comparison in the Car category. As shown in Table \ref{table:pepfe}, our simple yet effective PE-PFE design yields 1.9 point gains in Success and 0.7 point improvement in Precision. As shown in Figure \ref{fig:PE-loss}, the design of PE-PFE leads to lower loss values, enabling the network to find better parameters and achieve superior performance. 

% \subsection{Modality-aware Transformer-based Backbone} 
% % The original design of the computation distribution across stages in ResNet was largely empirical. The heavy “res4” stage was meant to be compatible with downstream tasks like object detection, where a detector head operates on the 14×14 feature plane. Swin-T, on the other hand, followed the same principle but with a slightly different stage compute ratio of 1:1:3:1. For larger Swin Transformers, the ratio is 1:1:9:1. Following the design, we adjust the number of blocks in each stage from (3, 4, 6, 3) in ResNet-50 to (3, 3, 9, 3), which also aligns the FLOPs with Swin-T. This improves the model accuracy from xx\% to xx\%. Notably, researchers have thoroughly investigated the distribution of computation , and a more optimal design is likely to exist. In this section, we design a series of 2D backbones, ranging from 3DTrackNet-Tiny with light weight to 3DTrackNet-Large with high performance, for different demands. Building upon the previous design principles, we propose our 3DTrackNet-Tiny, Small, Base and Large models.

% Recent studies~\cite{tian2022fully, zhou2023fastpillars, LKUnet} have pointed out that the backbone designs commonly employed in image domain~\cite{simonyan2014very, resnet, swin, convnext} are sub-optimal for point cloud or depth images due to significant modality differences between RGB images and LiDAR point clouds. Particularly, backbone design in image domain tends to utilize more block layers in later stages to extract high-level semantic features for perception. For instance, ResNet-50\cite{resnet} takes 6 residual blocks in the 3rd stage while the 1st stage uses 3 blocks for feature extraction. Similarly, Swin-Transformer~\cite{swin} adopts 9 blocks in the 3rd stage while only 1 block is used in the 1st stage. However, we think that these design choices for distributing computations across stages were largely empirical and may not be well-suited for LiDAR point clouds. Unlike RGB images, LiDAR can capture spatial distances and shapes of objects. This means that rich and accurate geometric information of objects is already explicitly encoded in point cloud. Therefore, we assume that instead of allocating excessive computational resources to model object geometries in later stages like ResNet/Swin-Transformer in RGB images, we propose reallocating more computational resources to the early stages to effectively incorporate the geometric information carried by raw point clouds.

% \begin{table}[h]
% \centering
% \caption{Impact of varying block quantities in the four stages of the backbone on the final results. \textbf{Bold} denotes the best performance.}\label{table:template}
% \resizebox{0.9\linewidth}{!}{
% \begin{tabular}{c|c|c|c}\toprule[.02cm]
% Blocks Number &GFLOPs & Success & Precision \\
% \hline \hline
% $\left[ 3, 4, 6, 3 \right]$ (SMAT\cite{smat}\footnotemark[3])   & 0.37  & 68.9  & 79.6 \\
% \midrule
% $\left[2, 2, 6, 2 \right]$   & 0.29  & 25.7  & 34.9 \\
% $\left[1, 1, 9, 1 \right]$   & 0.29  & 53.1  & 56.2 \\
% \midrule
% $\left[1, 1, 1, 1 \right]$  & 0.14  & 69.5  & 80.1 \\
% \midrule
% $\left[2, 1, 1, 1 \right]$   & 0.16  & 70.3  & 80.6   \\
% \rowcolor{gray!55}
% $\left[3, 1, 1, 1 \right]$    & \textbf{0.18}(\textbf{-0.19})  & \textbf{72.1}(\textbf{+3.2})  & \textbf{82.1} (\textbf{+2.5}) \\ 
% $\left[4, 1, 1, 1 \right]$  & 0.21  & 68.7  & 78.9 \\ 
% \midrule
% $\left[1, 2, 1, 1 \right]$    & 0.16  & 70.1  & 80.7   \\
% $\left[1, 3, 1, 1 \right]$   & 0.18  & 69.7  & 80.6   \\ 
% $\left[1, 4, 1, 1 \right]$ & 0.20  & 69.4  & 79.4 \\
% \midrule
% $\left[1, 1, 2, 1 \right]$  & 0.16  & 68.4  & 78.8   \\
% $\left[1, 1, 3, 1 \right]$  & 0.18  & 70.0  & 80.8   \\ 
% $\left[1, 1, 4, 1 \right]$ & 0.20  & 71.0  & 81.8 \\
% \midrule
% $\left[1, 1, 1, 2 \right]$   & 0.15  & 68.0  & 78.3   \\
% $\left[1, 1, 1, 3 \right]$  & 0.17  & 68.1  & 78.4   \\ 
% $\left[1, 1, 1, 4 \right]$   & 0.18  & 69.3  & 80.0   \\ 
% \bottomrule
% \end{tabular}
% }

% \vspace{-2mm}
% \label{fig:backbone}
% \end{table}

% To validate the aforementioned hypothesis for transformer-based backbone, we systematically study computation allocation by adjusting the stage compute ratio in the transformer-based backbone of SMAT~\cite{smat}. It is worth noting that the setting of SMAT has the same depth number as ResNet-50, with a stage compute ratio of $[3, 4, 6, 3]$. As shown in Table \ref{fig:backbone}, we used the SMAT backbone as the baseline and varied the number of depth blocks from 0 to 4 with a stride of 1 in each stage. From the results, we can find that the performance is quite sensitive to the capacity of early stage 1, while being less sensitive to the later stages (2, 3, 4). This confirmed that allocating more computational resources to the early stages is beneficial for enabling the network to better capture the geometric information carried by the raw point clouds. Based on this observation, we set the stage compute ratio of the four stages to $[3, 1, 1, 1]$. It is worth noting that with this depth blocks setting, our modality-aware transformer backbone network achieved promising performance improvements in terms of 3.2 point in Success and 2.5 point in Precision metric, while significantly reducing the computational cost by half the GFLOPs compared to the baseline method (from 0.37 to 0.18). 

% \textbf{Differences with Previous Study.} Our results differ significantly from previous studies~\cite{tian2022fully,zhou2023fastpillars}, which were focused on LiDAR-based object detection tasks using CNN architecture with local receptive fields. In contrast, we focus on 3D SOT tasks within local search area and design a transformer architecture with global receptive fields. Therefore, by allocating more computational resources to the 1st stage, our network is able to capture the enough global-aware geometric information of the input point cloud. This is different with CNN-based backbone, which require more computational resources allocated to both the 1st and 2nd stages. As a result, our modality-aware transformer-based backbone design proves to be more effective.



% %我们的动机/flops为标准，探索更高效的pillar-based 3D SOT任务。


% % \subsection{Quantization-Aware Pillar Encoder Design.} 
% % QA-Pillar


% % The Quantization-Aware Pillar Encoder (QA-Pillar) design is aimed at enhancing the efficiency and robustness of feature representation for point cloud data. Building upon traditional pillar-based feature extraction, this encoder introduces a quantization step that discretizes point cloud features at predefined quantization levels. This quantization process not only alleviates the computational load of the model but also improves its adaptability to the sparsity of point clouds. With quantized point cloud features, the QA-Pillar is more effective in capturing critical geometric information of the target object while mitigating the impact of noise on tracking performance. Furthermore, this design enables the model to optimize computational resources while maintaining a high level of feature expressiveness. Experimental results demonstrate that the QA-Pillar significantly enhances the accuracy and stability of tracking across various scenarios, particularly in situations with sparse or noisy point cloud data.

% % \subsection{Scalable Transformer-based Backbone}


% % \textbf{Exploring Stage Ratio by Computation Reallocation.}


% % \begin{table*}[t]%Car
% % \caption{Comparison of PillarTrackNet with model scales from  small, base to large. }
% % \centering
% % \begin{tabular}{c|c|c|c|c|c}\toprule[.02cm]
% % Model & Channels  &GFLOPs & $\#$Params (M) & Success & Precision \\
% % \toprule
% % PillarTrackNet-S   & [ 32, 64, 120, 256  ] & 0.06  & 1.93 &70.9  &81.2\\
% % PillarTrackNet-B    & [ 48, 96, 240, 384 ] & 0.11  & 4.89 &71.3 &82.0\\
% % PillarTrackNet-L   & [ 64, 128, 320, 512 ]  & 0.18  & 8.6 &72.1 &82.1\\
% % \bottomrule
% % \end{tabular}
% % \label{table:template}
% % \end{table*}

% % \textbf{The Impact of Pillar Size}
% % %pillar size
% % In our research on PillarTrackNet, we conducted an in-depth investigation into the impact of pillar size on the representation of point cloud features and tracking performance, while considering its compatibility with the backbone architecture design. Although smaller pillar sizes offer finer spatial resolution, they may lead to performance degradation when paired with an incompatible backbone architecture, as it may not effectively process high-resolution inputs. Conversely, larger pillar sizes, while simplifying computations, can result in the loss of critical local features, especially in scenarios requiring detailed feature extraction. Our experimental findings reveal a delicate balance between pillar size selection and backbone design, indicating that there is an optimal range of pillar sizes for specific backbone architectures to achieve better tracking performance. This discovery underscores the necessity to consider the interplay between pillar size, backbone architecture, and overall tracking strategy when designing 3D point cloud processing systems.

% \subsection{Activation Function Selection for Point Cloud}

% \begin{equation}
% \begin{aligned}
%  % f(x) = x \Phi(x) = x \left( 1 + \exp(-x^2) \right)^{-\frac{1}{2}}\\
% GeLU(x)=\frac{1}{2} x\left(1+\frac{2}{\sqrt{\pi}} \int_{0}^{\frac{x}{\sqrt{2}}} e^{-\eta^{2}} d \eta\right)
% \end{aligned}
% \label{equ:gelu}
% \end{equation}

% \begin{equation}
% \begin{aligned}
% ReLU(x) = \max(0, x)
% \end{aligned}
% \label{equ:relu}
% \end{equation}
% \vspace{-2mm}
% \begin{equation}
% \begin{aligned}
% LeakyReLU(x) = \begin{cases} 
% x & \text{if } x > 0, \\
% \alpha x & \text{if } x \leq 0.
% \end{cases}
% \end{aligned}
% \label{equ:leaky-relu}
% \end{equation}

% There is a discrepancy between the choice of activation functions natural language processing (NLP) and vision architectures. Rectified Linear Unit (ReLU)\cite{agarap2018deep} is extensively used in convolutional networks (ConvNets) due to its simplicity and efficiency. With the Transformer\cite{vaswani2017attention} merging, Gaussian Error Linear Unit (GELU)\cite{hendrycks2016gaussian} is considered as a smoother variant of ReLU and has been employed in state-of-the-art Transformer models, such as Google's BERT \cite{devlin2018bert}, OpenAI's GPT-3 \cite{brown2020language}, and Vision Transformers \cite{swin,vit}, demonstrating superior performance across various language and vision tasks. However, unlike image or text data, point cloud input data contains negative values that represent corresponding geometric property. We assume that directly applying ReLU or GELU activation functions to point clouds would suppress the negative values and result in information loss. To address this issue, we explored the Leaky Rectified Linear Unit (LeakyReLU)\cite{maas2013rectifier}, which can address the issue of neuron death and preserve more information within the range of values less than zero. As shwon in Eq. \ref{equ:gelu},\ref{equ:relu},\ref{equ:leaky-relu} The GELU and ReLU functions exhibit saturation behavior when the input values are less than zero, effectively reducing the information content. In contrast, the LeakyReLU function preserves the negative range of input values, enabling the retention of valuable information.

% \begin{table}[h]
% \caption{ Influence of different activation functions on Car category.\textbf{Bold} denotes the best result}
% \centering
% \begin{tabular}{c|c|c}\toprule[.02cm]
% PFE Method & Success & Precision\\
% \toprule%3463-0.1-bs16*4-pillarvfe
% GELU (SMAT\cite{smat}\footnotemark[3])    & 68.9  & 79.6\\
% ReLU   & 69.9  & 80.7   \\
% % ELU   & 68.4  & 80.0   \\
% % PReLU   & 68.6  & 78.8   \\
% \textbf{LeakyReLU}    & \textbf{71.2 (+2.3)} & \textbf{81.8 (+2.2)}  \\ 
% \bottomrule
% \end{tabular}
% \label{table:act}
% \vspace{-2mm}
% \end{table}

% \begin{figure}[h]
% \centering
% \includegraphics[width=0.8\linewidth]{figures/LOSS_Activation.pdf}\vspace{-2mm}
% % Reduce the figure size so that it is slightly narrower than the column.
% \caption{\textbf{The impact of different activation functions on the reduction of the Epoch Loss.}Inparticular, the LeakyReLU activation function has shown a more pronounced decrease in loss compared to the other two functions under consideration.}
% \label{fig:leakyreu}
% \vspace{-3mm}
% \end{figure}

% Therfore, we simply replace the GeLU activatation function in SMAT with LeakyReLU function. As shown in Tab \ref{table:act} and Figure \ref{fig:leakyreu}, using LeakyReLU function has better performance (+2.3 in Success and 2.2 in Precision) and lower loss value than other functions, highlighting the significant impact of activation function choice on 3D single object tracking tasks based on point cloud modality.


% % \textbf{Pretrain Strategy.}
% % %explore pretrain: pillarnest.
% % In the context of 3D Single Object Tracking, a pre-trained backbone network provides an optimized weight initialization that significantly accelerates the learning process and enhances the model's ability to recognize features within point cloud data. This pre-training strategy leverages the rich visual features learned from large-scale datasets such as ImageNet\cite{imagenet}, enabling more efficient feature extraction and target tracking in 3DSOT tasks. PillarNeSt\cite{pillarnest}, a network architecture specifically designed for point cloud data, has been pre-trained on ImageNet\cite{imagenet}, thereby equipping it with the capacity to effectively process point cloud data.

% % To further optimize PillarNeSt\cite{pillarnest} for our 3DSOT task, we implemented a weight initialization strategy that ensures the model inherits effective feature representations from the pre-training phase. We preserved the core pillar encoder and decoder structure of PillarNeSt\cite{pillarnest} and fine-tuned the network's channel and layer configurations to cater to the characteristics of point cloud data. This approach allows our model to maintain the advantages of pre-trained weights while adapting to the sparsity and irregularity of point cloud data.

% % By utilizing the pre-trained backbone, our 3DSOT model is capable of rapidly acquiring new tasks and achieving real-time, high-precision target tracking. This strategy not only enhances the model's generalization capability but also contributes to an improvement in tracking performance.


% \begin{table*}[h]
% \caption{Overall performance comparison on the KITTI dataset. The best two results are highlighted in \textcolor{red}{red}, \textcolor{blue}{blue}.}
% \centering
% \resizebox{\linewidth}{!}{
% \begin{tabular}{c|c|c|c|c|cc|cc}
% 		\hline
% 		\multirow{2}{*}{Method} & \multirow{2}{*}{Publication} & \multirow{2}{*}{Modality} & \multirow{2}{*}{Paradigm} &\multirow{2}{*}{View} & \multicolumn{2}{c|}{Mean-by class} & \multicolumn{2}{c}{Mean-by frame} \\
%   & & & & & Success    & Precision & Success    & Precision\\\hline 
% 	$M^2$-Track ~\cite{mmtrack} & CVPR 2022 & LIDAR &Motion &Point &61.9 & \textcolor{blue}{80.2} &60.6  &\textcolor{blue}{80.1}  \\ \hline
% 		SC3D\cite{sc3d} & CVPR 2019 &\multirow{13}{*}{LIDAR}  & \multirow{13}{*}{Similarity} &Point & 35.4 & 53.3 & 31.2 & 48.5 \\
%   P2B\cite{p2b} & CVPR 2020 &  & &Point &39.5 & 53.9 & 42.4 & 60.0 \\
%   3D-SiamRPN\cite{fang20203d} & IEEE Sensors J &  & &Point &43.8 & 58.6 &46.6 & 64.9 \\
%   MLVSNet\cite{MLVSNet} & ICCV2021 &  & &Point &44.1 & 60.3 & 45.7 & 66.7 \\
%   BAT\cite{bat}  & ICCV 2021 &  & &Point &47.2 & 65.1 & 51.2 & 72.8\\
%   PTT\cite{ptt}  & IROS 2021 &  & &Point &48.4 & 63.4& 55.1 & 74.2\\
%   LTTR\cite{lttr}  & BMVC 2021 &  & &Voxel &50.0 & 67.4& 48.7 & 65.8\\
%   V2B\cite{v2b}  &NeurIPS 2021  &  & &Point+Voxel &52.4 & 65.6 &58.4  &75.2 \\
%   PTTR\cite{zhou2022pttr}  & CVPR 2022 &  & &Point &58.4 &77.8 & 57.9 & 78.1\\
%   CMT\cite{guo2022cmt}  &  ECCV 2022&  & &Point &57.2 &76.0 &59.4  &77.6 \\
%   STNet\cite{hui2022stnet}  &  ECCV 2022&  & &Point &\textcolor{blue}{63.4}&\textcolor{red}{81.4} &\textcolor{blue}{61.3}  &\textcolor{blue}{80.1} \\
%         C2FT\cite{c2ft}  &  RAL 2022&  & &Point &51.6 &67.7 &57.2 &76.4 \\
%         MLSET\cite{mlset}  &  RAL 2023&  & &Point &54.2 &68.9 &59.6  &78.4  \\
%         % PTTR++\cite{pttr_journal} &  TPAMI 2024&  & &Point+Pillar & \textcolor{red}{63.8} & \textcolor{blue}{81.0} & \textcolor{blue}{63.9} & \textcolor{red}{82.8}  \\ \hline
%         % \rowcolor{gray!55}
%         % \textbf{PillarTrack-S}  & Ours &  & &Pillar &61.3 &77.2 &\textcolor{blue}{64.4}  &80.6 \\
%         % \rowcolor{gray!55}
%         % \textbf{PillarTrack-B}  & Ours &  & &Pillar &62.3 &77.6 &\textcolor{blue}{64.4}  &80.8 \\
%         \hline
%         \rowcolor{gray!30}
%         SMAT\cite{smat} & RAL 2022 &  & &Pillar &56.7 &76.1 & 60.4 & 79.5 \\
%         \rowcolor{gray!55}
%         \textbf{PillarTrack}  & Ours &  & &Pillar &\textcolor{red}{63.7} \textbf{+7.0} &78.9 \textbf{+2.8} &\textcolor{red}{65.3} \textbf{+4.9}  &\textcolor{red}{82.2} \textbf{+2.7}\\
% 		\hline
%     \end{tabular}
%     }
% \label{tab:evaluation_car}
% \end{table*}

% \begin{table*}[t]
% \caption{Detailed per-class performance on the KITTI dataset. The best two results are highlighted in \textcolor{red}{red}, \textcolor{blue}{blue}.}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{c|cc|cc|cc|cc}
% \toprule[.05cm]
% \multirow{2}{*}{Method} & \multicolumn{2}{c|}{Car-6424} & \multicolumn{2}{c|}{Pedestrian-6088} & \multicolumn{2}{c|}{Van-1248} & \multicolumn{2}{c}{Cyclist-308} \\
% &  Success    & Precision   & Success    & Precision   & Success    & Precision   & Success    & Precision \\ \hline \hline
% $M^2$-Track~\cite{mmtrack} & 64.8 & 79.2 & \textcolor{blue}{57.6} &\textcolor{blue}{83.6} & 50.4 & 64.8 & \textcolor{blue}{74.9} & 93.3          \\ \hline
% SC3D~\cite{sc3d}    & 41.3       & 57.9        & 18.2       & 37.8        & 40.4       & 47.0        & 41.5       & 70.4                \\
% P2B~\cite{p2b}& 56.2& 72.8 & 28.7 & 49.6 & 40.8  & 48.4  & 32.1 & 44.7  \\
% 3D-SiamRPN\cite{fang20203d} & 58.2 & 76.2 & 35.2 & 56.2 & 45.7 & 52.9 & 36.2 & 49.0         \\
% MLVSNet\cite{MLVSNet} &56.0 & 74.0 & 34.1 & 61.1 & 52.0 & 61.4 & 34.3 & 44.5 \\
% BAT~\cite{bat} & 60.5       & 77.7        & 42.1       & 70.1        & 52.4       & 67.0& 33.7       & 45.4                \\
% PTT~\cite{ptt} & 67.8       & 81.8        & 44.9       & 72.0        & 43.6       & 52.5        & 37.2       & 47.3                \\
% LTTR~\cite{lttr} & 65.0       & 77.1        & 33.2       & 56.8        & 35.8       & 45.6        & 66.2      & 89.9                \\
% V2B~\cite{v2b}  & 70.5       & 81.3        & 48.3       & 73.5        & 50.1       & 58.0        & 40.8       & 49.7                \\
% PTTR~\cite{zhou2022pttr}  & 65.2       & 77.4        & 50.9       & 81.6        & 52.5& 61.8        & 65.1       & 90.5\\
% CMT\cite{guo2022cmt}   & 70.5       & 81.9        & 49.1       & 75.5        & 54.1& 64.1        & 55.1       & 82.4\\
% STNet~\cite{hui2022stnet}  &\textcolor{blue}{ 72.1}&\textcolor{blue}{84.0}& 49.9& 77.2& \textcolor{red}{58.0}& \textcolor{red}{70.6}& 73.5 & \textcolor{blue}{93.7}\\
% % TAT~\cite{tat} & \textcolor{blue}{72.2}       & 83.2        & 57.4       & 84.4        & \textcolor{red}{58.9}       & 69.2 & \textcolor{blue}{74.2}       & \textcolor{blue}{93.9} \\0

% C2FT~\cite{c2ft}  & 67.0& 80.4& 48.6& 75.6& 53.4& \textcolor{blue}{66.1}& 38.0& 48.7\\
% MLSET~\cite{mlset} & 69.7& 81.0& 50.7& 80.0& \textcolor{blue}{55.2}& 64.8& 41.0& 49.7\\
% % PTTR++\cite{pttr_journal} &\textcolor{blue}{73.4} & \textcolor{blue}{84.5} & 55.2 &84.7& 55.1 & 62.2 & 71.6 & 92.8\\ \hline
% % 新增PillarTrackNet行
% % \rowcolor{gray!55}
% % \textbf{PillarTrack-S (Ours)} & 71.9 & 82.3 &\textcolor{red}{61.1} &\textcolor{red}{84.9} &40.0 &48.3 &72.1 &93.1 \\
% % \rowcolor{gray!55}
% % \textbf{PillarTrack-B (Ours)} &\textcolor{blue}{73.8} &\textcolor{blue}{84.7} &58.7 &82.4 &41.2 &49.2 &\textcolor{blue}{75.5} &\textcolor{blue}{94.0} \\
% \hline
% \rowcolor{gray!30}
% SMAT~\cite{smat}  & 71.9& 82.4& 52.1& 81.5& 41.4& 53.2& 61.2& 87.3\\ 
% \rowcolor{gray!55}
% \textbf{PillarTrack (Ours)} &\textcolor{red}{74.2} \textbf{+2.3} &\textcolor{red}{85.1} \textbf{+2.7}&\textcolor{red}{59.7}\textbf{+7.6} &\textcolor{red}{84.7} \textbf{+3.2}&43.4 \textbf{+2.0}&51.7 \textbf{--} &\textcolor{red}{77.4} \textbf{+16.2}&\textcolor{red}{94.2} \textbf{+6.9}\\
% \bottomrule
% \end{tabular}
% }
% \label{tab:kitti}
% \vspace{-3mm}
% \end{table*}

% \section{Experiments}
% %In this study, we conducted training and evaluation for our 3D single object tracking task using the KITTI dataset \cite{kitti}. However, due to the absence of annotation information for the KITTI test set, we followed the established practices from previous research \cite{sc3d,p2b} by solely utilizing the training set for both training and evaluating our tracking model. The KITTI dataset consists of 21 video sequences encompassing eight distinct object categories. For the training phase, we selected scenes 0 to 16 as our training data, scenes 17 to 18 for model validation, and scenes 19 to 20 for testing purposes.  Similar to prior works such as \cite{sc3d,p2b,ptt}, our primary focus was on rigid car tracking, and we performed ablation studies specifically on the KITTI dataset. Additionally, we conducted extended experiments involving three other target categories (Pedestrian, Van, Cyclist) to comprehensively evaluate the performance of our method for tracking non-rigid objects (Pedestrian) on the KITTI dataset.
% \textbf{ KITTI Dataset.} 
% We conduct training and evaluating for our task using the KITTI \cite{kitti} datasets. We follow the same setting in baseline model\cite{smat} to divide the sequences into training,
% validation, and testing splits, where 0-16 for training, 17-18
% for validation and 19-20 for testing.
% %split the training and val set. During the training phase, we selected scenes 0 to 16 as our training data, scenes 17 to 18 for model validation, and scenes 19 to 20 for testing. Similar to baseline mode\cite{smat}, we mainly focused on rigid car tracking and performed ablation studies on KITTI. We also conducted extended experiments with other three target categories (Pedestrian, Van, Cyclist) to comprehensively evaluate the performance of our method for non-rigid objects (Pedestrian) tracking on KITTI.

% \textbf{ NuScenes Dataset.} 
% The NuScenes\cite{nuscenes} dataset comprises 1000 scenes, which are allocated into 700/150/150 scenes for training, validation, and testing, respectively. Each scene is populated with approximately 300,000 points and is accompanied by comprehensive 360-degree viewpoint annotations. In our research, we adhere to the dataset configuration established by Open3DSOT\cite{mmtrack} for the training and evaluation of our methodology. We also conduct a comparative analysis with the baseline model\cite{smat}to evaluate the efficacy and superiority of our designs.


% \textbf{Evaluation metrics.}
% We use One-Pass Evaluation (OPE) \cite{kristan2016novel} to measure Success and Precision. The Success measure the 3D IoU between the predicted box and the ground truth box, the Precision measures the AUC of the distance error between the center of the predicted and ground truth box.
% %to assess the efficacy of our tracking approach. The Success metric is determined by calculating the Intersection over Union (IoU) between the predicted bounding box and the ground truth bounding box, which serves as a measure of tracking accuracy. The Precision metric evaluates the performance by analyzing the Area Under the Curve (AUC) of the distance error between the centroids of the predicted and ground truth bounding boxes. Collectively, these metrics provide a holistic evaluation framework that enables an objective assessment of the tracking algorithm's performance.

% \textbf{Implementation details.}
% We follow our baseline model\cite{smat} and employ PVTv2-b2 \cite{pvtV2} as backbone, adhering to its original configuration. The specific settings include a head number of [1, 2, 5, 8], a depth configuration of [3, 1, 1, 1], the expansion ratio for the feed-forward layer set to [8, 8, 4, 8] and a channel number configuration of [64, 128, 320, 512]. In KITTI dataset, we set [0.1, 0.1, 4] meters as pillar size and a search area of [-3.2, -3.2, -3, 3.2, 3.2, 1] meters for the car category. In nuScenes dataset, we set [0.075, 0.075, 8] meters as pillar size and a search area of [-3.2, -3.2, -5, 3.2, 3.2, 3] meters for the car category. Additionally, the LeakyReLU activation is employed with a negative slope value of 0.01.
% %Within the Cross-FPN module, both the output channel and feed-forward channel are set to 256, with the cross-attention heads and attention layers each configured to 8. In the decoder, the head number and layer number are both set to 8, and the feedforward channel is set to 2048. 
% %In iterative experiments, we further explored two distinct backbone architectures: ResNet (including ResNet18 and ResNet34), in addition to the initially adopted PVTv2-b2. Based on these networks, we conducted a series of ablation studies to analyze the impact of varying depth configurations, channel numbers, decoder structures, activation functions, pillar encoding methods, and point cloud encoding strategies on model performance and inference latency. The specific experimental settings are as follows: depth configurations ranged from [1, 1, 1, 1] to [10, 10, 2, 2], channel numbers expanded from [32, 64, 120, 256] to [96, 192, 380, 768], and pillar sizes were adjusted from [0.05, 0.05, 4] to [0.1, 0.1, 4]. Activation functions were compared between ReLU, GeLU and LeakyReLU. Pillar encoding methods included both the initial PillarVFE and the experimental Quantization-Aware Pillar. Additionally, we conducted corresponding experimental settings for non-rigid objects, such as pedestrians, to evaluate the model's performance in handling such objects. Through these systematic ablation and combination experiments, we continuously optimized the model architecture to achieve optimal tracking performance and inference efficiency.

% \textbf{Training details.} On the KITTI dataset, we train PillarTrack with AdamW\cite{loshchilov2017decoupled} optimizer with an initial learning rate of 0.0001, a weight decay of 0.05, and a batch size of 16 on a NVIDIA 3090 GPU. The total number of training epochs was set to 72. For the NuScenes dataset, the training was conducted over 18 epochs, with a learning rate decay by a factor of 10 at epoch 14.



% \begin{table*}[!t]
% \vspace{0.2in}
% \renewcommand\tabcolsep{3pt}
% \scriptsize
% \centering
% \begin{tabular}{c|c|cc|cc|cc|cc|cc|cc|cc}
% \toprule[.05cm]
% \multirow{2}{*}{Method} & \multirow{2}{*}{Paradigm} & \multicolumn{2}{c|}{Car-64159} & \multicolumn{2}{c|}{Pedestrian-33227} & \multicolumn{2}{c|}{Truck-13587} & \multicolumn{2}{c|}{Trailer-3352} & \multicolumn{2}{c|}{Bus-2953} &\multicolumn{2}{c|}{Mean by class} & \multicolumn{2}{c}{Mean by frame} \\
% &                           & Success    & Precision   & Success    & Precision   & Success     & Precision    & Success      & Precision    & Success    & Precision & Success    & Precision & Success    & Precision  \\ \hline \hline
% $M^2$-Tracker~\cite{mmtrack}  & Motion & \textcolor{red}{55.85} &\textcolor{red}{65.09}   &       32.10      &  \textcolor{blue}{60.92}  &\textcolor{red}{57.36} &\textcolor{red}{59.54}      &\textcolor{blue}{  57.61}  &\textcolor{red}{58.26}   &  \textcolor{red}{51.39}  &\textcolor{red}{51.44} &\textcolor{red}{50.86}&\textcolor{red}{59.05} &\textcolor{red}{49.23}&\textcolor{red}{62.73} \\ \hline
% SC3D~\cite{sc3d} & \multirow{8}{*}{Similarity}    &   22.31         &    21.93  &11.29   &12.65    & 30.67  &27.73    &35.28  & 28.12  & 29.35  &24.08  & 25.78&22.90 &20.70&20.20            \\
% P2B~\cite{p2b} &   & 38.81  & 43.18  &  28.39 & 52.24  & 42.95 & 41.59&  48.96     &  40.05    &  32.95 & 27.41 &38.41 &40.90 &36.48&45.08  \\
% PTT~\cite{ptt-journal} &   & 41.22  & 45.26  &  19.33 & 32.03  & 50.23 & 48.56&  51.70     &  46.50    &  39.40 & 36.70 &40.38 &41.81 &36.33&41.72  \\
% BAT~\cite{bat} &   &40.73 & 43.29 & 28.83 & 53.32   &45.34&   42.58   &52.59   &44.89  &35.44   & 28.01 &40.59 &42.42  &38.10&45.71  \\ 
% GLT-T~\cite{glt} &   & 48.52  & 54.29  &  31.74 & 56.49  & 52.74 & 51.43&  57.60     &  52.01    &  44.55 & 40.69 &47.03 &50.98 &44.42&54.33  \\
% PTTR~\cite{zhou2022pttr} &   &\textcolor{blue}{ 51.89}  &\textcolor{blue}{ 58.61}  &  29.90 & 45.09  & 45.30 & 44.74&  45.87     &  38.36    &  43.14 & 37.74 &43.22 &44.91  &44.50&52.07  \\
% % CMT~\cite{guo2022cmt} &     &  47.00         &    51.70  &-   &-    &52.50   &52.50    & \textcolor{red}{62.00}  & \textcolor{blue}{58.20}   &  \textcolor{blue}{46.30}  & \textcolor{blue}{42.90}  & -&- &-&-            \\
% % V2B~\cite{v2b} &     &  \textcolor{blue}{ 54.40}        &    \textcolor{blue}{ 59.70 } &30.10   &55.40    & 53.70 &51.10    &54.90  & 43.70  & -  &-  & -&- &-&-            \\
% % STNet~\cite{sc3d} &     &   32.2         &    36.1  &19.1   &27.2    & 22.3  &27.73    &35.28  & 28.12  & 29.35  &24.08  & 25.78&22.90 &20.70&20.20            \\
% % C2FT~\cite{c2ft} &     &   40.80         &    43.80  &-   &-    & 48.40  &46.60    &58.50  &51.80  & 40.50  &36.60  &- &- &-&-            \\
% % MLSET~\cite{mlset} &     &   53.20         &   58.30  & \textcolor{blue}{33.20}  &58.60    & 54.30  &52.50    &-  & -  & 53.10  &40.90  &- &- &-&-            \\
% % PTTR++~\cite{pttr_journal} &     &   59.96         &    66.73  &32.49   &50.50    & 59.85  &61.20    &54.51  & 50.28  & 53.98  &51.22  & 52.16&55.97 &51.86&60.63            \\
% \hline
% \rowcolor{gray!25}
% SMAT~\cite{smat} &   & 43.51 & 49.04 & \textcolor{blue}{32.27}  &60.28 & 44.78& 44.69&37.45 & 34.10  &39.42 & 34.32 &39.49 &44.49 &40.20&50.92            \\ 
% \rowcolor{gray!50}
% \textbf{PillarTrack} &  & 47.12 & 57.72 &\textcolor{red}{34.18} &\textcolor{red}{64.93}& \textcolor{blue}{54.82}& \textcolor{blue}{54.41}&\textcolor{red}{57.70} &\textcolor{blue}{54.63} &\textcolor{blue}{44.68} &\textcolor{blue}{40.73} & \textcolor{blue}{47.70}& \textcolor{blue}{54.48} &\textcolor{blue}{44.59} &\textcolor{blue}{58.86}\\ \hline
% Improvement &  & \textbf{+3.61} & \textbf{+8.68} & \textbf{+1.91} &\textbf{+4.65} & \textbf{+10.04}&\textbf {+9.72}& \textbf{+17.25}&\textbf{+20.53} &\textbf{+5.26} & \textbf{+6.41}  &\textbf {+8.21} &\textbf {+9.99}  &\textbf {+4.39} &\textbf {+7.94}\\
% \toprule[.05cm]
% \end{tabular}
% \caption{Performance comparison on the NuScenes dataset. The best two results are highlighted in \textcolor{red}{red}, \textcolor{blue}{blue}.}
% \label{tab:nuscenes}
% \vspace{-0.3in}
% \end{table*}

% \subsection{Quantitative results on KITTI.}
% As shown in Table \ref{tab:evaluation_car} and \ref{tab:kitti}, the proposed PillarTrack demonstrates significant performance improvements compared to the baseline method (SMAT \cite{smat}). Specifically, PillarTrack achieved a performance improvement of 7.0\% \/ 2.8\% and 4.9\% \/ 2.7\% in Success and Precision metrics in terms of mean by-class and mean-by frame setting, respectively. 

% In the categories of the Car, Pedestrian, Van, and Cyclist, PillarTrack outperformed SMAT by 2.3\%, 7.6\%, 2.0\%, and 16.2\% in Success, respectively. These improvements can be attributed to the effective designs of PillarTrack. Firstly, PE-PFE module could stabilize network training without information loss. Secondly, the modality-aware transformer-basde backbone focuses on capturing more geometric information from point clouds and enhance the feature representation capability of pillars. Lastly, LeakyReLU activation retains more information and help network optimization. Besides, PillarTrack also surpassed the motion-based method MMTrack~\cite{mmtrack} in the categories of Car, Pedestrian, and Cyclist, achieving state-of-the-art performance on the KITTI dataset. However, for Van, our method only has 43.4\% in Success. We believe there are two main reasons for this. Firstly, the point clouds of vans are concentrated on the object surfaces, and after pillar encoding, they lack distinctive geometric features, making them more challenging to track accurately. Secondly, the limited number of training samples for the Van category may have constrained the model's performance, as it might not have captured the full range of variations and characteristics exhibited by vans in the real world.


% \subsection{Quantitative results on NuScenes.}
% As illustrated in Table \ref{tab:nuscenes}, our PillarTrack achieves the second-best performance across the five categories on the nuScenes dataset. Compared to previous methods, M2-Tracker\cite{mmtrack} adopts a different motion-based paradigm for object tracking, demonstrating superior results compared to the similarity-based paradigm. Meanwhile, our PillarTrack attains the best results among the similarity-based methods. Furthermore, compared to the baseline method\cite{smat}, PillarTrack has demonstrated significant improvements in each category. Specifically, PillarTrack has enhanced the mean class-wise and frame-wise Success and Precision metrics by 8.21\% / 9.99\% and 4.39\% / 7.94\%, respectively. In terms of Success for each category, PillarTrack achieves notable improvements of 3.61\% for Car, 1.91\% for Pedestrian, 10.04\% for Truck, 17.25\% for Trailer, and 5.26\% for Bus. Importantly, the Truck and Trailer categories demonstrate significantly enhanced performance compared to baseline. However, such improvements were not observed in the Van category in the KITTI dataset. We attribute this to two reasons: (1) The KITTI dataset only provides front-view annotations. Under the front-view perspective, the model is constrained to learn feature representations specific to the truck from a single viewpoint, which limits the acquisition of comprehensive geometric information about the Van. As a result, the Siamese network based on appearance matching struggles to capture the key geometric information of the Van. Conversely, the NuScenes dataset provides 360-degree surround view point cloud data with corresponding annotations. This enables superior learning of both appearance and geometric representations, leading to significant performance enhancement by effectively utilizing multi-view point cloud data. (2) The KITTI dataset contains a limited number of annotated van samples (1248), whereas the NuScenes dataset offers a larger sample size (13587/3352). Within our effective framework design, this facilitates richer feature representation learning, leading to performance improvements. Besides, our performance is slightly lower than that of PTTR on Car category. We think this is because PTTR utilizes both point-based and pillar-based representations to encode the input point cloud, resulting in superior performance, particularly in terms of the Success metric.


% % %only car 

% \subsection{Visualization results.}
% \begin{figure*}[!t] % h:here 当前位置 % b bottom % t top % p 浮动
%     \centering
%     \includegraphics[width=\linewidth]{figures/visual.pdf}
%     \caption{Visualization results comparison of our PillarTrack and SMAT on the point cloud sequences of Car, Pedestrian and Cyclist categories.}
%     \label{figure:compare}
%     \vspace{-4mm}
% \end{figure*}
% To comprehensively evaluate the performance of our method, particularly its capability to handle point clouds of varying sparsity, we conduct visualization on the different category, encompassing both sparse and dense scenes. Through comparative experiments on the initial frame and subsequent sequences, our method demonstrated superior tracking accuracy in both sparse and dense point cloud environments compared to the baseline SMAT method, highlighting ours enhanced adaptability and robustness. In the Cyclist category, our method was able to consistently track the target, whereas SMAT occasionally lost the target. For the Pedestrian category, our method maintained stable tracking from the outset, while SMAT failed to accurately identify the target initially. The visualization results in Figure 5 further substantiate the effectiveness and superior performance of our method across various scenarios.


% \subsection{Running Speed}
% We calculated the average running time of all test frames for car to measure PillarTrack's speed. PillarTrack model achieved 27 FPS on a single NVIDIA 3080 GPU, while baseline model SMAT has a 18.2 FPS in the inference
% phase. We did not introduce extra computational parameters, and we further reduced the computational overhead on the backbone while increasing the model's performance. This once again demonstrates the effectiveness of our PillarTrack. Furthermore, our proposed PillarTrack can leverage quantization techniques\cite{lidar-ptq,nagel2021white} to accelerate the runtime. We leave this problem for future research.


% \section{CONCLUSIONS}

% In this work, we explored PillarTrack, a pillar-based 3D single-object tracking framework that decreases computation overhead while improving performance. The framework introduces a Pyramid-type Encoding Pillar Feature Encoder (PE-PFE) and a modality-aware Transformer-based backbone, and a simply replacement of activation function. Our extensive experiments on the KITTI dataset demonstrate PillarTrack's superior performance, achieving an better trade-off between speed and accuracy. Based on above designs and its efficiency, We hope to inspire the community to rethink the design of network for 3D single object tracking based on point clouds. We will open source our code. 

% %\addtolength{\textheight}{-12cm}   % This command serves to balance the column lengths
%                                   % on the last page of the document manually. It shortens
%                                   % the textheight of the last page by a suitable amount.
%                                   % This command does not take effect until the next page
%                                   % so it should come on the page before the last. Make
%                                   % sure that you do not shorten the textheight too much.
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % \begin{figure*}[htbp]
% % \centering
% % \includegraphics[width=1.0\textwidth]{fig/num_blocks.pdf}\vspace{-2mm}
% % % Reduce the figure size so that it is slightly narrower than the column.
% % \caption{\textbf{Impact of varying block quantities in the four stages of the backbone on the final results.} Each subfigure corresponds to a different stage of the backbone. Subfigure $(a)\sim(d)$ shows the effect of changing the number of blocks in Stage $1\sim4$, respectively. As can be seen, different stages show varying sensitivity to the number of blocks utilized.}
% % \label{fig:num_blocks}
% % \end{figure*}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % \section*{APPENDIX}
% % Appendixes should appear before the acknowledgment.
% % \section*{ACKNOWLEDGMENT}
% % The preferred spelling of the word ÒacknowledgmentÓ in America is without an ÒeÓ after the ÒgÓ. Avoid the stilted expression, ÒOne of us (R. B. G.) thanks . . .Ó  Instead, try ÒR. B. G. thanksÓ. Put sponsor acknowledgments in the unnumbered footnote on the first page.
% % %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % References are important to the reader; therefore, each citation must be complete and correct. If at all possible, references should be commonly available publications.
% \bibliographystyle{unsrt}
% \bibliography{refenrences}
% \end{document}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


